Scaling Ensemble Distribution Distillation to Many Classes with Proxy Targets

Ensembles of machine learning models yield improved system performance as well as robust and interpretable uncertainty estimates; however, their inference costs may often be prohibitively high. \emph{Ensemble Distribution Distillation} is an approach that allows a single model to efficiently capture both the predictive performance and uncertainty estimates of an ensemble. For classification, this is achieved by training a Dirichlet distribution over the ensemble members' output distributions via the maximum likelihood criterion. Although theoretically principled, this criterion exhibits poor convergence when applied to large-scale tasks where the number of classes is very high. In our work, we analyze this effect and show that the Dirichlet log-likelihood criterion classes with low probability induce larger gradients than high-probability classes. This forces the model to focus on the distribution of the ensemble tail-class probabilities. We propose a new training objective that minimizes the reverse KL-divergence to a \emph{Proxy-Dirichlet} target derived from the ensemble. This loss resolves the gradient issues of Ensemble Distribution Distillation, as we demonstrate both theoretically and empirically on the ImageNet and WMT17 En-De datasets containing 1000 and 40,000 classes, respectively.

==> apn.tex <==
\section{Emulating Ensembles via Autoregressive Prior Networks}
While ensemble methods give a theoretically meaningful approach to modelling uncertainty, they can be prohibitively computationally expensive for many real applications. This is even more true for large auto-regressive models like Transformers~\cite{attentionisallyouneed,vgg-transformer}. One approach 

Here we consider how to generalize distribution distillation to auto-regressive structured predictions models, yielding Sequence Ensemble Distributions Distillation (SEnD$^2$). Unlike, ensembles of classification models, which can be interpreted as samples from implicit conditional distribution over discrete output distributions, ensembles of auto-regressive models can be interpreted as samples of prefix-trees samples from a distribution over prefix-trees conditioned on the input $\bm{x}f$. Unfortunately, it is not possible to explicitly parameterize such a distribution in practice. However, it was shown in ~\cite{malinin-structured-2020}, ensemble-combination should be done at the token, not sequence level for improved prediction and uncertainty estimation. The reason being that an 'atomic' component of an auto-regressive model is an unstructured prediction of the next token $y_l$ given a context $\bm{y}_{<l}$ and input $\bm{x}$, and all further prefix-tree structure arises out of the combination of these predictions. Ensembles of auto-regressive models can therefore be interpreted a samples from a distribution over output distributions conditioned on the input and the context.
\begin{empheq}{align}
\big\{{\tt P}(y_l | \bm{y}_{<l}, \bm{x} ; \bm{\theta}^{(m)} )\big\}_{m=1}^M \rightarrow&\ {\tt p}(\bm{\pi}_l | \bm{y}_{<l},\bm{x};\bm{\hat \phi})
\end{empheq}

% One approach to decreasing the computational load is \emph{knowledge distillation} or \emph{ensemble distillation}~\cite{hinton2015distilling}. Here one or more models are distilled into a single, potentially smaller model. Knowledge Distillation has also been applied to structured predictions models~\cite{sequence-knowledge-distillation}, where auto-regressive models were distilled by maximizing the probability of the predicted hypotheses of a teacher model. A range of other models considered minimizing the KL-divergence between the conditional distributions of the teacher model (or mean conditional distributions) and a student model~\cite{sequence-distillation,ctc-distillation,asr-distillation1,asr-distillation2}. 
% \begin{empheq}{align}
% \begin{split}
% \mathcal{L}_{\tt SEnD}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\  -\mathbb{E}_{{\tt \hat p}(\bm{x},\bm{y}_l)}\Big[{\tt KL}\big[\mathbb{E}_{{\tt q}(\bm{\theta})}[{\tt  p}(y_l|\bm{y}_{<l},\bm{x},\bm{\theta})]\ ||\ {\tt p}(y_l | \bm{y}_{<l}, \bm{x};\bm{\phi})\big] \Big]
% \end{split}
% \label{eqn:end-loss1}
% \end{empheq}

We now consider how to emulate an ensemble of auto-regressive models using a Prior Networks. Consider an \emph{autoregressive} Prior Network (APN) ${\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \theta})$ which yields a distribution over output distributions $\bm{\pi}_l =\ \left[{\tt P}(y_l=\omega_1),\cdots,{\tt P}(y_l=\omega_K) \right]^{{\tt T}}$ at every time-step. This model is defined as follows:
Given this model, Token-level BMA, unlike sequence-level BMA, can be straightforwardly emulated as follows:
\begin{empheq}{align}
\begin{split}
{\tt P}(\bm{y}|  \bm{x}, \mathcal{D}) =&\ \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \bm{\theta})\Big] \approx \prod_{l=1}^L \mathbb{E}_{{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \phi})}[{\tt P}(y_l|\bm{\pi}_l)] =\ {\tt P}(\bm{y}| \bm{x}; \bm{\hat \phi})
\end{split}\label{eqn:emulation}
\end{empheq}

In this work we consider a model which yields a Dirichlet distribution at each time-step:
\begin{empheq}{align}
\begin{split}
{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \phi}) =&\ {\tt Dir}(\bm{\pi} | \bm{\hat \alpha}^{(l)}),\quad \bm{\hat \alpha}^{(l)} =\ \bm{f}(\bm{y}_{<l},\bm{x};\bm{\hat \phi}),\quad \hat \alpha_c^{(l)} > 0,\ \hat \alpha_0^{(l)} = \sum_{c=1}^K \hat \alpha_c^{(l)}
\end{split}
\label{eqn:DPN1}
\end{empheq}



Let's examine how given this model we can obtain measures of sequence-level \emph{total} and \emph{knowledge} uncertainty. \emph{Total Uncertainty} will be given by the sequence-level entropy.
\begin{empheq}{align}
\begin{split}
\mathcal{\hat H}\big[{\tt P}(\bm{y}| \bm{x}; \bm{\hat \phi})\big] =&\ \frac{1}{L} \mathbb{E}_{{\tt P}(\bm{y}| \bm{x}; \bm{\hat \phi})}\big[{\tt P}(\bm{y}| \bm{x}; \bm{\hat \phi})\big] =\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l}| \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat H}\big[{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \bm{\hat \phi})\big] \big]
\end{split}\label{eqn:product-of-expectations}
\end{empheq}

% \begin{empheq}{align}
% \begin{split}
% \mathcal{\hat I}[\bm{y},\bm{\theta}|\bm{x}]  =&\ \frac{1}{L}\sum_{l=1}^L\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\theta})}\big[{\tt KL}[{\tt P}(y_l| \bm{y}_{<l}, \bm{x};  \bm{\theta}\|{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \mathcal{D})]\big]\big]  \\
% \approx&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x};  \mathcal{D})}\big[\mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt KL}[{\tt P}(y_l| \bm{y}_{<l}, \bm{x};  \bm{\theta}\|{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \mathcal{D})]\big]\big]  \\
% \approx&\   \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathbb{E}_{{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \theta})}\big[{\tt KL}[{\tt P}(y_l|\bm{\pi}_l)\| {\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \bm{\hat \phi}]\big]\big] \\
% =&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat I}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat I}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
% \end{split}\label{eqn:apn-sequence-mi}
% \end{empheq}
% \begin{empheq}{align}
% \begin{split}
% \mathcal{\hat K}[\bm{y},\bm{\theta}|\bm{x}]  \approx&\  \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x} \mathcal{D})}\big[\mathcal{\hat K}[y_l,\bm{\theta}|\bm{y}_{<l}, \bm{x}]\big] \\
% \approx&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat K}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat K}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
% \end{split}\label{eqn:apn-sequence-mi}
% \end{empheq}
% \begin{empheq}{align}
% \begin{split}
% \mathcal{\hat M}[\bm{y},\bm{\theta}|\bm{x}]  =&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \mathcal{D})}\big[\mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt KL}[{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \mathcal{D}\|{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \bm{\theta})]\big]\big]  \\
% \approx&\   \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathbb{E}_{{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \theta})}\big[{\tt KL}[{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \bm{\hat \phi}\|{\tt P}(y_l|\bm{\pi}_l)]\big]\big] \\
% =&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat M}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat M}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
% \end{split}\label{eqn:apn-sequence-mkl}
% \end{empheq}

\begin{empheq}{align}
\begin{split}
\mathcal{\hat I}[\bm{y},\bm{\theta}|\bm{x}] \approx&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat I}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat I}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
\end{split}\label{eqn:apn-sequence-mi}
\end{empheq}

\begin{empheq}{align}
\begin{split}
\mathcal{\hat K}[\bm{y},\bm{\theta}|\bm{x}] \approx&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat K}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat K}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
\end{split}\label{eqn:apn-sequence-mi}
\end{empheq}

\begin{empheq}{align}
\begin{split}
\mathcal{\hat M}[\bm{y},\bm{\theta}|\bm{x}] \approx&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{x}; \bm{\hat \phi})}\big[\mathcal{\hat M}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}]\big] =\ \mathcal{\hat M}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]
\end{split}\label{eqn:apn-sequence-mkl}
\end{empheq}



\subsection{Monte-Carlo Approximation}

\begin{empheq}{align}
\begin{split}
\mathcal{\hat H}^{(S)}\big[{\tt P}(\bm{y}| \bm{x}; \bm{\hat \phi})\big] \approx&\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L \mathcal{\hat H}\big[{\tt P}(y_l| \bm{y}_{<l}, \bm{x}; \bm{\hat \phi})\big],\quad   \bm{y}_{<l}^{(s)} \in  \bm{y}^{(s)} \sim {\tt P}(\bm{y} | \bm{x}; \bm{\hat \phi})
\\
=&\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L\Big[-\sum_{k=1}^K \frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\ln\frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\Big]
\end{split}\label{eqn:product-of-expectations}
\end{empheq}

\begin{empheq}{align}
\begin{split}
&\mathcal{\hat I}^{(S)}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]  =\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L \mathcal{\hat I}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}],\quad   \bm{y}_{<l}^{(s)} \in  \bm{y}^{(s)} \sim {\tt P}(\bm{y} | \bm{x}; \bm{\hat \phi}) \\
&\ = \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L\Big[-\sum_{k=1}^K \frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\ln\frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}} + \sum_{k=1}^K \frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\big(\psi(\hat \alpha_k^{(sl)}+1) - \psi(\hat \alpha_0^{(sl)}+1)\big)\Big]
\end{split}\label{eqn:apn-sequence-mi}
\end{empheq}

\begin{empheq}{align}
\begin{split}
\mathcal{\hat K}^{(S)}[\bm{y},\bm{\pi}_{1:L}|\bm{x}]  \approx&\  \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L \mathcal{\hat K}[y_l,\bm{\pi}_l|\bm{y}_{<l}^{(s)}, \bm{x}],\quad   \bm{y}_{<l}^{(s)} \in  \bm{y}^{(s)} \sim {\tt P}(\bm{y} | \bm{x}; \bm{\hat \phi})\\
=&\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L \frac{K-1}{\hat \alpha_0^{sl}}
\end{split}\label{eqn:apn-sequence-mi}
\end{empheq}



\begin{empheq}{align}
\begin{split}
 \mathcal{\hat M}^{(S)}[\bm{y},\bm{\pi}_{1:L}|\bm{x}] \approx&\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L \mathcal{\hat M}[y_l,\bm{\pi}_l|\bm{y}_{<l}, \bm{x}],\quad   \bm{y}_{<l}^{(s)} \in  \bm{y}^{(s)} \sim {\tt P}(\bm{y} | \bm{x}; \bm{\hat \phi})\\
=&\ \frac{1}{SL}\sum_{s=1}^S\sum_{l=1}^L\Big[-\sum_{k=1}^K \frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\big(\psi(\hat \alpha_k^{(sl)}) - \psi(\hat \alpha_0^{(sl)})\big) +\sum_{k=1}^K \frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\ln\frac{\hat \alpha_k^{(sl)}}{\hat \alpha_0^{(sl)}}\Big] 
\end{split}\label{eqn:apn-sequence-mkl}
\end{empheq}

==> distillation_structured_uncertainty.tex <==
\section{Distillation for Structured Prediction}

\begin{eqnarray*}
{\cal D}
%% =\left\{\{{\bm x}^{(1)},y^{(1)}\},\ldots,{\bm x}^{(N)},y^{(N)}\}\right\}
=
\left\{\{{\bm x}^{(i)},y^{(i)}\}\right\}_{i=1}^N
; \:\:\:\:
y^{(i)}\in\{\omega_1,\ldots,\omega_K\}
\end{eqnarray*}
In terms of standard notation given the training data ${\cal D}$ training can be expressed as
\begin{eqnarray}
{\overline{\bm\theta}} = 
= 
\argmax_{\bm\theta}\left\{
\sum_{i=1}^N
\log\left({\tt P}(y^{(i)}|\bm{x}^{(i)}; {{\bm{\theta}}})\right)
\right\}
\end{eqnarray}
The labels, $y$ from the joint distribution are now discarded, and the posteriors frome the trained model are used to estimate the distilled model parameters ${\hat{\bm\theta}}$
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}; {{\bm{\theta}}})}
\big]
\right\}
\end{eqnarray}
where
\begin{eqnarray}
{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}; {{\bm{\theta}}})}
\big] = 
\sum_{k=1}^K{\tt P}(y=\omega_k|{\bm x}^{(i)}; {\overline{\bm{\theta}}})\log
\left(
\frac{{\tt P}(y=\omega_k|{\bm x}^{(i)}; {\overline{\bm{\theta}}})}
{{\tt P}(y=\omega_k|{\bm x}^{(i)};{\bm\theta})}
\right)
\end{eqnarray}
When the data is now structured, for example tasks such as speech recognition, speech synthesis and machine translation the joint distribution of the data is more complicated as there are now observations sequences and label sequences. The data distribution can be expressed as~\footnote{Of course $T$ and $L$ vary, but for simplicity this is ignored for notational simplicity.} ${\tt p}_{\tt tr}({\bm x}_{1:T},y_{1:L})$. Again only samples from the true distribution 
\begin{eqnarray*}
{\cal D}
%% =\left\{\{{\bm x}^{(1)},y^{(1)}\},\ldots,{\bm x}^{(N)},y^{(N)}\}\right\}
=
\left\{\{{\bm x}^{(i)}_{1:T},y^{(i)}_{1:L}\}\right\}_{i=1}^N
; \:\:\:\:
y^{(i)}\in\{\omega_1,\ldots,\omega_K\}
\end{eqnarray*}
Again this data can be used to train a standard sequence model with parameters ${\overline{\bm\theta}}$. One optimal difference is that the simple (conditional) maximum likelihood training for unstructured data can use minimum Bayes risk training with an appropriate sequence loss function.  The original implementation of knowledge distillation, or teacher-student training, for this form of model used a simple per sample approximation
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N\sum_{j=1}^T{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}_j; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}_j; {{\bm{\theta}}})}
\big]
\right\}
\end{eqnarray}
Effectively this has ignored the problem as a sequence problem. Sequence teacher-student training, sequence distillation, aims to address this problem by considering posterior distributions of complete sequences, compressed into a lattice ${\cal L}$ generated from model ${\overline{\bm\theta}}$ for the $i-th$ sample, ${\cal L}|\bm{x}^{(i)}_{1:T}; {\overline{\bm{\theta}}}$. The expression then becomes
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N{\tt KL}\big[
{\cal L}|\bm{x}^{(i)}_{1:T}; {\overline{\bm{\theta}}}
\big|\big|
{\cal L}|\bm{x}^{(i)}_{1:T}; {\bm{\theta}}
\big]
\right\}
\end{eqnarray}

For these approaches there is no assumption that the complexity of the models is consistent between ${\overline{\bm\theta}}$ and ${\hat{\bm\theta}}$. This distillation can be used to simplify the complexity of the model, yielding speed and memory advantages.

The second application of distillation is to distill an ensemble of models into a single model. Applying standard ensemble distillation
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N\sum_{m=1}^M{\tt KL}\big[
{\tt p}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}}^{(m)})
\big|\big|
{\tt p}(y|\bm{x}^{(i)}; {\bm{\theta}})
\big]
\right\}
\end{eqnarray}
where the ensemble of models comprises parameters, $\left\{{\overline{\bm\theta}}^{(m)}\right\}_{m=1}^M$.  As previously mentioned this has ignored the diversity associated with the model. To address this problem ensemble distribution distillation can be used. Here the distribution of the predictions in the ensemble is modelled. Denote the prediction of sample ${\bm x}^{(i)}$ using model ${\overline{\bm\theta}}^{(m)}$ as
\begin{eqnarray}
{\bm\pi}^{(mi)} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)}) \\
\vdots\\
{\tt P}(y=\omega_K|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)}) 
\end{array}
\right]; 
\:\:\:\:
{\bm\pi}^{(mi)} \sim {\tt p}_{\pi}({\bm x}^{(i)})
\end{eqnarray}
To model the ensemble distribution these samples can then be used for training the model
\begin{eqnarray}
{\hat{\bm\theta}} = 
\argmin_{\bm\theta}\left\{
\sum_{i=1}^N
{\tt KL}\big[
{\tt p}_{\pi}(\bm{x}^{(i)})
\big|\big|
{\tt p}_{\pi}(\bm{x}^{(i)}; {\bm{\theta}})
\big]
\right\}
\approx
\argmax_{\bm\theta}\left\{
\sum_{i=1}^N
\sum_{m=1}^M
\log\left(
{\tt p}_{\pi}({\bm\pi}^{(mi)} | \bm{x}^{(i)}; {\bm{\theta}})
\right)
\right\}
\end{eqnarray}
This form of model, associated with distributions over distributions, is a prior network. This has the same form as density networks, networks that predict the parameters of parametric distributions, but the form here is a distribution over distributions. Thus
\begin{eqnarray*}
{\tt p}_{\pi}({\bm\pi}^{(mi)} | \bm{x}^{(i)}; {\bm{\theta}})
= {\tt Dir}({\bm\pi}^{(mi)}; {\cal F}_\alpha(\bm{x}^{(i)}; {\bm{\theta}}))
\end{eqnarray*}
where ${\cal F}_\alpha(\bm{x}^{(i)}; {\bm{\theta}})$ yields the appropriate Dirichlet distribution parameters.

Extending this form of distribution to handle structured data is non-trivial. It is possible to extend the notation above to handle lattices
\begin{eqnarray}
{\cal L}^{(mi)} = 
{\cal L}|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)};
\:\:\:\:
{\cal L}^{(mi)} \sim {\tt p}_{\cal L}({\bm x}^{(i)})
\end{eqnarray}
The challenge is to decide on the appropriate parametric form for ${\tt p}_{\cal L}({\bm x}^{(i)};{\bm\theta})$.

\section{Sequence Distribution Distillation}
The simplest approach to a distribution over the lattice~\footnote{The initial form considered here is a prefix-tree not a lattice.} is to make an additional conditional independence assumption: the distribution over the predicted word distributions is only dependent on the history of words to that point. Thus consider adding a new arc ${\cal A}$ to the lattice having taken word sequence $w_{1:\tau-1}=w_1,\ldots,w_{\tau-1}$ where $w_\tau\in\{\omega_k\}_{k=1}^K$. Initially just consider the scenario where only the word-id information is  considered (so duration and score are not considered). The task is to get the distribution over the predictions for word $w_\tau$. Consider
\begin{eqnarray*}
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{1:\tau-1};{\bm\theta})
\end{eqnarray*}
where
\begin{eqnarray}
{\bm\pi}_{\tau} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|w_{1:\tau-1}) \\
\vdots\\
{\tt P}(y=\omega_K|w_{1:\tau-1}) 
\end{array}
\right]
\end{eqnarray}

Consider the following form
\begin{eqnarray}
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{1:\tau-1};{\bm\theta})
\approx
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{\tau-1},{\bm\alpha}_{\tau-1};{\bm\theta})
= {\tt Dir}({{\bm\pi}}_{\tau};{\cal F}_\alpha(w_{\tau-1},{\bm\alpha}_{\tau-1};{\bm\theta})
= {\tt Dir}({{\bm\pi}}_{\tau};{\bm\alpha}_{\tau})
\end{eqnarray}
This effectively replaces the standard PMF prediction from an RNN-LM, with a Dirichlet distribution prediction. Following this logic through
\begin{eqnarray}
{\cal F}_\alpha(w_{\tau},{\bm\alpha}_{\tau};{\bm\theta}) \approx
{\cal F}_\alpha(w_{\tau},{\bm h}_{\tau};{\bm\theta}); \:\:\:\:
{\bm h}_{\tau} = {\cal F}_{\tt h}(w_{\tau-1},{\bm h}_{\tau-1};{\bm\theta})
\end{eqnarray}
This form of model can be trained in the same fashion as standard LMs, but now using the distributions that result from an ensemble if language models. Let 
\begin{eqnarray}
{\bm\pi}^{(m)}_{\tau} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|w_{1:\tau-1};{\bm\theta}^{(m)}) \\
\vdots\\
{\tt P}(y=\omega_K|w_{1:\tau-1};{\bm\theta}^{(m)}) 
\end{array}
\right]
\end{eqnarray}
The optimisation criterion then becomes
\begin{eqnarray}
{\hat{\bm\theta}} = \argmax_{{\bm\theta}}\left\{
\sum_{\tau=1}^L\sum_{m=1}^M\log\left(
{\tt p}_{\pi}({\bm\pi}^{(m)}_{\tau}|w_{1:\tau-1};{\bm\theta})
\right)
\right\}
\end{eqnarray}



==> ensemble_uncertainty.tex <==
\section{Uncertainty Estimation via Ensembles}\label{sec:ensembles}
%%%%FLOW!!!!!!%%%%

In this work we take a Bayesian viewpoint on ensembles, as it yields an elegant probabilistic framework within which interpretable uncertainty estimates can be obtained. The core of the Bayesian approach is to treat the model parameters $\bm{\theta}$ as random variables and place a prior  ${\tt p}(\bm{\theta})$ over them to compute a posterior ${\tt p}(\bm{\theta}|\mathcal{D})$ via Bayes' rule:
\begin{empheq}{align}
\begin{split}
  {\tt p}(\bm{\theta}|\mathcal{D}) &= \frac{{\tt p}(\mathcal{D}|\bm{\theta}){\tt p}(\bm{\theta})}{{\tt p}(\mathcal{D})}
\end{split}
\label{eqn:bayesposterior}
\end{empheq}
However, exact Bayesian inference is intractable for neural networks. It is therefore necessary to consider an explicit or implicit approximation ${\tt q}(\bm{\theta})$ to the true posterior ${\tt p}(\bm{\theta}|\mathcal{D})$ to generate an ensemble of models. A number of different approaches to generating an ensemble of models have been developed, such as Monte-Carlo Dropout~\cite{Gal2016Dropout}, DeepEnsembles~\cite{deepensemble2017}, and Stochastic Weight Averaging Gaussian (SWAG)~\cite{maddox2019simple}. A full overview is available in~\cite{ashukha2020pitfalls, trust-uncertainty}. 

Consider an ensemble of models $\{{\tt P}(y | \bm{x}; \bm{\theta}^{(m)})\}_{m=1}^M$ sampled from an approximate posterior ${\tt q}(\bm{\theta})$, where each model captures an \emph{unstructured} mapping $\bm{x} \rightarrow y$, where $\bm{x} \in \mathcal{R}^D$ and $y \in \{\omega_1,\cdots,\omega_K\}$. Each of the models ${\tt P}(y|\bm{x}, \bm{\theta}^{(m)})$ yields a \emph{different} estimate of \emph{data uncertainty}. Uncertainty in predictions due to \emph{knowledge uncertainty} is expressed as the level of spread, or `disagreement', of models in the ensemble~\cite{malinin-thesis}. The \emph{predictive posterior} of the ensemble is obtained by taking the expectation with respect to the models in the ensemble:
\begin{empheq}{align}
\begin{split}
{\tt P}(y | \bm{x}, \mathcal{D}) =&\  \mathbb{E}_{{\tt p}(\bm{\theta}|\mathcal{D})}\big[{\tt P}(y | \bm{x} ; \bm{\theta}) \big] \\
\approx&\ \frac{1}{M}\sum_{m=1}^M {\tt P}(y | \bm{x}; \bm{\theta}^{(m)}),\ \bm{\theta}^{(m)} \sim {\tt q}(\bm{\theta})
\end{split}
\end{empheq}
The entropy of the predictive posterior will be an estimate of \emph{total uncertainty} in predictions:
\begin{empheq}{align}
\mathcal{H}\big[{\tt P}(y |  \bm{x}, \mathcal{D})\big] =&\  \mathbb{E}_{{\tt P}(y |  \bm{x},  \mathcal{D})}\big[ -\ln {\tt P}(y | \bm{x},  \mathcal{D}) \big] 
\end{empheq}
\emph{Total uncertainty} in the prediction is due to both \emph{data uncertainty} and \emph{knowledge uncertainty}. However, for tasks such as misclassification detection considering the log-likelihood score assigned by the predictive posterior to a particular class can yield superior performance as it is more sensitive to the prediction made~\cite{malinin-thesis}:
\begin{empheq}{align}
\begin{split}
\text{SCR} =&\ \ln{\tt P}(y = \hat \omega| \bm{x}, \mathcal{D})
\end{split}
\end{empheq}

In certain situations, such as active learning~\cite{batchbald} and out-of-distribution input detection, it is desirable to evaluate uncertainty in predictions due to \emph{knowledge uncertainty}. The sources of uncertainty can be decomposed by considering the \emph{mutual information} between the model parameters $\bm{\theta}$ and the prediction $y$~\cite{mutual-information}:
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{I}\big[y, \bm{\theta} | \bm{x}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}} =&\ \underbrace{\mathcal{H}\big[{\tt P}(y |  \bm{x}, \mathcal{D})\big]}_{\text{Total Uncertainty}} \\
- &  \underbrace{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y | \bm{x}; \bm{\theta})]\big]}_{\text{Expected Data Uncertainty}}
\end{split}\label{eqn:mi}
\end{empheq}
This is expressed as the difference between the entropy of the predictive posterior and the expected entropy of each model in the ensemble. The former is a measure of \emph{total uncertainty}, while the later is a measure of \emph{expected data uncertainty}. Their difference will be measure of spread of the ensemble and an estimate of \emph{knowledge uncertainty}. It is also possible to consider the \emph{expected pairwise KL-divergence} between models in an ensemble as an alternative measure of ensemble diversity:
\begin{empheq}{align}
\begin{split}
\mathcal{K}[y, \bm{\theta}] =&\ \mathbb{E}_{{\tt q}(\bm{\theta}){\tt q}(\bm{\tilde \theta})}\big[{\tt KL}[{\tt P}(y|\bm{x},\bm{\theta})||{\tt P}(y|\bm{x},\bm{\tilde \theta}) ]\big] \\
=&  \underbrace{-\sum_{y} \mathbb{E}_{{\tt q}(\bm{\theta})}[{\tt P}(y|\bm{x}, \bm{\theta})]\mathbb{E}_{{\tt q}(\bm{\tilde \theta})}[\ln{\tt P}(y|\bm{x}, \bm{\tilde \theta}]}_{\text{Total Uncertainty}}\\
- &  \underbrace{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y | \bm{x}; \bm{\theta})]\big]}_{\text{Expected Data Uncertainty}}
\end{split}
\label{eqn:epklbayes}
\end{empheq}
where ${\tt q}(\bm{\theta})={\tt q}(\bm{\tilde \theta})$. This measure is an upper bound on the mutual information and also allows \emph{total uncertainty} to be decomposed into \emph{knowledge uncertainty} and \emph{data uncertainty}~\cite{malinin-thesis}. Notably, only estimates of \emph{total uncertainty} differ, while the estimate of \emph{data uncertainty} provided by both decompositions is the same. 







% First, let's consider the entropy of as single model in the ensemble at an input $\bm{x}$:
% \begin{empheq}{align}
% \begin{split}
%  \mathcal{H}\big[{\tt P}(y | \bm{x}; \bm{\theta})\big]
% =&\ \mathbb{E}_{{\tt P}(y |  \bm{x}; \bm{\theta})}\big[ -\ln {\tt P}(y | \bm{x}; \bm{\theta}) \big] 
% \end{split}
% \end{empheq}
% This will be an estimate of \emph{data uncertainty}, or uncertainty due to the natural complexity of the data~\cite{malinin-thesis}.

==> sendd.tex <==
\section{Sequence Ensemble Distribution Distillation}\label{sec:sendd}

Having established how to emulate an ensemble of autoregressive models using an Autoregressive Prior Network, we now examine how to carry out Sequence Ensemble Distribution Distillation.

Typically, Ensemble Distribution Distillation is done in a two-step fashion. First, a transfer dataset is formed. This can either be the original training dataset or using context deriving from the B-best beam-search hypotheses of the teacher $\{\bm{\hat y}^{(b)}\}_{b=1}^B$ within the beam $\mathcal{B}$. Previous work on sequence-level knowledge distillation show that the latter yields superior results. However, we will re-evaluate this in the context of SEnD$^2$.
\begin{empheq}{align}
\begin{split}
\mathcal{D}_{\tt ens} =&\ \Big\{\bm{x}^{(i)}, \big\{\{\bm{\pi}_l^{(1:M)}, \bm{\hat y}_{<l}\}_{l=1}^{L_i}\big\}^{(i)} \Big\}_{i=1}^{B\cdot N} =\ {\tt \hat p}(\bm{x},\bm{\hat y}_{<l}, \bm{\pi}_l)
\end{split}
\end{empheq}
Here the transfer dataset is equivalent to the empirical distribution ${\tt \hat p}(\bm{x},\bm{\hat y}_{<l}, \bm{\pi}_l)$ which figures in the expressions below. Secondly, given the transfer dataset, the likelihood of the predictions of each model in the ensemble, given the B-best contexts, for each input $\bm{x}$, is maximized under the Dirichlet prior:
\begin{empheq}{align}
\begin{split}
\mathcal{L}_{\tt SEnD^2}^{NLL}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\  \mathbb{E}_{{\tt \hat p}(\bm{x},\bm{\hat y}_{<l})}\big[\mathbb{E}_{{\tt \hat p}(\bm{\pi}_l|\bm{\hat y}_{<l},\bm{x})}[-\ln{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\phi}) ] \big] %\\
%=&\ \mathbb{E}_{{\tt \hat p}(\bm{x},\bm{\hat y}_{<l})}\big[{\tt KL}\big[{\tt \hat p}(\bm{\pi}_l|\bm{\hat y}_{<l},\bm{x})\|{\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\phi})\big] \big] +Z
\end{split}
\label{eqn:endd-nll-loss}
\end{empheq}

Unfortunately, as will be shown in the next section, this naive approach does not perform well in practice due to several issues.

\textbf{Mediator Dirichlet} The distribution of the ensemble's predictions on the simplex is unlikely to be Dirichlet-distributed. 

\begin{empheq}{align}
\big\{{\tt P}(y_l | \bm{y}_{<l}, \bm{x} ; \bm{\theta}^{(m)} )\big\}_{m=1}^M \rightarrow&\ {\tt p}(\bm{\pi}_l | \bm{\beta}_l(\bm{x},\bm{y}_{<l})) \rightarrow {\tt p}(\bm{\pi}_l | \bm{y}_{<l},\bm{x};\bm{\hat \phi})
\end{empheq}

\begin{empheq}{align}
\begin{split}
\mathcal{L}_{\tt SEnD^2}^{KL}(\bm{\phi},\mathcal{D}_{\tt ens}) =\  \mathbb{E}_{{\tt \hat p}(\bm{x},\bm{\hat y}_{<l})}\big[{\tt KL}\big[{\tt \hat p}\big(\bm{\pi}_l| \bm{\beta}_l(\bm{x},\bm{y}_{<l})\big)\|{\tt p}\big(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\phi}\big)\big] \big] \\
=\  \ln\Gamma(\beta_0)- \sum_{k=1}^K\ln\Gamma(\beta_k) +\sum_{k=1}^K\ln\Gamma(\alpha_k) - \ln\Gamma(\alpha_0) + \sum_{k=1}^K(\beta_k-\alpha_k)\big(\psi(\beta_k) - \psi(\beta_0)\big)% \\
%=\ \sum_{k=1}^K\ln\Gamma(\alpha_k) - \ln\Gamma(\alpha_0) + -\sum_{k=1}^K\alpha_k\big(\psi(\beta_k) - \psi(\beta_0)\big)  + Z
\end{split}
\label{eqn:endd-kl-loss}
\end{empheq}

\begin{empheq}{align}
 \bm{\beta}_l(\bm{x},\bm{y}_{<l}) = \bm{\hat \pi}_l \cdot \beta_0,\quad \bm{\hat \pi}_l = \frac{1}{M}\sum_{m=1}^M\bm{\pi}_l^{(m)},\ \beta_0^1 = \frac{K-1}{\mathcal{K}(y_l,\bm{\theta}|\bm{x})},\ \beta_0^2 = \frac{K-1}{2\mathcal{M}(y_l,\bm{\theta}|\bm{x})}
\end{empheq}

\begin{empheq}{align}
\mathcal{K}(y_l,\bm{\theta}|\bm{x}) &\ \frac{1}{M(M-1)}\sum_{m=1}^M\sum_{j=1}^M {\tt KL}[\bm{\pi}_l^{m}\|\bm{\pi}_l^{j}],\quad \mathcal{M}(y_l,\bm{\theta}|\bm{x}) =\ \frac{1}{M}\sum_{m=1}^M{\tt KL}[\bm{\hat \pi}_l\|\bm{\pi}_l^{m}]
\end{empheq}


\textbf{Aggregation Trick}
\begin{empheq}{align}
\begin{split}
\frac{\partial\mathcal{L}_{\tt SEnD^2}^{KL}}{\partial \alpha_k} =\  \psi(\alpha_k) - \psi(\alpha_0) - \big(\psi(\beta_k) - \psi(\beta_0)\big)
%=\ \sum_{k=1}^K\ln\Gamma(\alpha_k) - \ln\Gamma(\alpha_0) + -\sum_{k=1}^K\alpha_k\big(\psi(\beta_k) - \psi(\beta_0)\big)  + Z
\end{split}
\label{eqn:nll}
\end{empheq}

\begin{empheq}{align}
\begin{split}
\frac{\partial\mathcal{L}_{\tt SEnD^2}^{KL}}{\partial \alpha_k} =\  \psi(\sum_{k+1}^K\alpha_k) - \psi(\alpha_0) - \big(\psi(\sum_{k+1}^K\beta_k) - \psi(\beta_0)\big)
%=\ \sum_{k=1}^K\ln\Gamma(\alpha_k) - \ln\Gamma(\alpha_0) + -\sum_{k=1}^K\alpha_k\big(\psi(\beta_k) - \psi(\beta_0)\big)  + Z
\end{split}
\label{eqn:nll2}
\end{empheq}



\textbf{Length-scale adjustment}

\begin{empheq}{align}
\begin{split}
\frac{\partial T\mathcal{L}_{\tt SEnD^2}^{KL}}{\partial \alpha_k} =&\  \psi(\frac{\alpha_k}{T}) - \psi(\frac{\alpha_0}{T}) - \big(\psi(\frac{\beta_k}{T}) - \psi(\frac{\beta_0}{T})\big)
\approx\ \ln\frac{\hat \pi_k}{\pi_k^{\beta}} -\frac{T}{2}\Big(\frac{\alpha_0 - \alpha_k}{\alpha_k\alpha_0} -  \frac{\beta_0 - \beta_k}{\beta_k\beta_0}\Big)%,\quad \pi_k^\beta = \frac{\beta_k}{\beta_0}
%=\ \sum_{k=1}^K\ln\Gamma(\alpha_k) - \ln\Gamma(\alpha_0) + -\sum_{k=1}^K\alpha_k\big(\psi(\beta_k) - \psi(\beta_0)\big)  + Z
\end{split}
\label{eqn:nll3}
\end{empheq}

\textbf{Alternative Dirichlet Parameterization}

\begin{empheq}{align}
\begin{split}
\alpha_k =&\ \hat\pi_k \cdot \alpha_0,\quad \alpha_0 = e^{z_0},\  \bm{\hat \pi} = {\tt softmax}(\bm{z})
\end{split}
\label{eqn:nll3}
\end{empheq}


\begin{empheq}{align}
\begin{split}
\frac{\partial \alpha_k}{\partial z_k} =&\  (1-\hat \pi_k) \alpha_k,\quad \frac{\partial \alpha_k}{\partial z_0} = \alpha_k
\end{split}
\label{eqn:nll3}
\end{empheq}















% A crucial limitation of all knowledge distillation approaches is that information about the diversity of the ensemble, which is necessary for separation of uncertainties into \emph{knowledge uncertainty} and \emph{data uncertainty}, is lost in the process~\cite{malinin-endd-2019}. It has been shown that this separation is especially useful for structured uncertainty estimation~\cite{malinin-structured-2020}. However, a recent new approach to distillation, called Ensemble Distribution Distillation (EnD$^2$)~\cite{malinin-endd-2019}, solves this problem and allows distilling ensembles of classification models into a single model whilst preserving information about ensemble diversity. Here, an ensemble is interpreted as a set of samples from an \emph{implicit} conditional distribution over output distributions:
% \begin{empheq}{align}
% \begin{split}
% \big\{{\tt P}(y| \bm{x}^{*}, \bm{\theta}^{(m)} )\big\}_{m=1}^M \rightarrow& \big\{{\tt P}(y| \bm{\pi}^{(m)} )\big\}_{m=1}^M,\quad 
% \bm{\pi}^{(m)} \sim\  {\tt p}(\bm{\pi} | \bm{x}^{*}, \mathcal{D})
% \end{split}
% \end{empheq}
% It is possible to \emph{distribution-distill} the ensemble into a model ${\tt p}(\bm{\pi} | \bm{x};\bm{\hat \phi})$ which parameterizes an \emph{explicit} conditional distribution output distributions via a straightforward application of maximum-likelihood estimation.
% \begin{empheq}{align}
% \big\{{\tt P}(y | \bm{x} ; \bm{\theta}^{(m)} )\big\}_{m=1}^M \rightarrow&\ {\tt p}(\bm{\pi} | \bm{x};\bm{\hat \phi})
% \end{empheq}
%In~\cite{malinin-endd-2019} this explicit distribution over distributions was modelled using a neural network model which parameterizes the Dirichlet Distribution:
% \begin{empheq}{align}
% \begin{split}
% {\tt p}(\bm{\pi} | \bm{x};\bm{\hat \phi}) =&\ {\tt Dir}(\bm{\pi} | \bm{\hat \alpha}),\quad \bm{\hat \alpha} =\ \bm{f}(\bm{x};\bm{\hat \phi}),\quad \hat \alpha_c > 0,\ \hat \alpha_0 = \sum_{c=1}^K \hat \alpha_c
% \end{split}
% \label{eqn:DPN1}
% \end{empheq}
% However, as a single uni-model Dirichlet may be too restrictive and poorly capture the behaviour of an ensemble, we can also consider a model which yields a mixture of Dirichlet distributions:
% \begin{empheq}{align}
% \begin{split}
% {\tt p}(\bm{\pi}_l | \bm{y}_{<l}, \bm{x};\bm{\hat \phi}) =&\ \sum_{j=1}^J w_j\cdot{\tt Dir}(\bm{\pi} | \bm{\hat \alpha}^{(l,j)}) \\
% \big\{\{\bm{\hat \alpha}^{(l,j)}\}_{j=1}^J,\ \bm{w}^{(l)}\big\} =&\ \bm{f}(\bm{y}_{<l},\bm{x};\bm{\hat \phi}),\quad \hat \alpha_c^{(l,j)} > 0,\ w_j^{(l)} \geq 0, \sum_{j=1}^J w_j^{(l)}=1
% \end{split}
% \label{eqn:DPN1}
% \end{empheq}

% \begin{empheq}{align}
% \begin{split}
% \mathcal{L} =&\ \sum_{c=1}^K\ln\Gamma(\alpha_c)-\ln\Gamma(\alpha_0) - \sum_{c=1}^K(\alpha_c-1)\ln\pi_k \\
% =&\ \sum_{c=1}^K\ln\Gamma(\alpha_c)-\ln\Gamma(\alpha_0) - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[(\alpha_c - \frac{1}{2})\ln\alpha_c\big] -\big[(\alpha_0 - \frac{1}{2})\ln\alpha_0\big] - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[(\alpha_0\hat \pi_c - \frac{1}{2})\ln\alpha_0\hat \pi_c\big] -\big[(\alpha_0 - \frac{1}{2})\ln\alpha_0\big] - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[(\alpha_0\hat \pi_c - \frac{1}{2})\ln\alpha_0\hat \pi_c\big] -\big[(\alpha_0 - \frac{1}{2})\ln\alpha_0\big] - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[(\alpha_0\hat \pi_c - \frac{1}{2})(\ln\alpha_0+\ln\hat \pi_c)\big] -\big[(\alpha_0 - \frac{1}{2})\ln\alpha_0\big] - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[\alpha_0\hat \pi_c\ln\alpha_0 - \frac{1}{2}\ln\alpha_0 + \alpha_0\hat \pi_c\ln\hat \pi_c - \frac{1}{2}\ln\hat \pi_c \big] -\big[\alpha_0\ln\alpha_0 - \frac{1}{2}\ln\alpha_0\big] - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[+ \alpha_0\hat \pi_c\ln\hat \pi_c - \frac{1}{2}\ln\hat \pi_c\big]  + \frac{1-K}{2}\ln\alpha_0 - \alpha_0\sum_{c=1}^K\hat \pi_k\ln\pi_k + C \\
% =&\ \sum_{c=1}^K\big[\alpha_0\hat \pi_c\ln\frac{\hat \pi_c}{\pi_c} - \frac{1}{2}\ln\hat \pi_c\big]  + \frac{1-K}{2}\ln\alpha_0 + C \\
% =&\ \alpha_0{\tt KL}[\bm{\hat \pi}||\bm{\pi}] - \frac{1}{2}\sum_{c=1}^K\ln\hat \pi_c  + \frac{1-K}{2}\ln\alpha_0 + C \\
% \end{split}
% \label{eqn:endd-loss}
% \end{empheq}
% , and is is accomplished in two steps. Firstly, a \emph{transfer dataset} $\mathcal{D}_{\tt ens}= \{\bm{x}^{(i)}, \bm{\pi}^{(i,1:M)} \}_{i=1}^N \sim {\tt \hat p}(\bm{x},\bm{\pi})$ is composed of the inputs $\bm{x}^{(i)}$ from the original training set $\mathcal{D}=\{\bm{x}^{(i)},y^{(i)}\}_{i=1}^N$ and the categorical distributions $\{\bm{\pi}^{(i,1:M)}\}_{i=1}^N$ derived from the ensemble for each input. Secondly, given this transfer set, the model ${\tt p}(\bm{\pi} | \bm{x};\bm{\phi})$ is trained by minimizing the negative log-likelihood of each categorical distribution $\bm{\pi}^{(im)}$:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{L}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\  -\mathbb{E}_{{\tt \hat p}(\bm{x})}\big[\mathbb{E}_{{\tt \hat p}(\bm{\pi}|\bm{x})}[\ln{\tt p}(\bm{\pi} | \bm{x};\bm{\phi}) ] \big]
% \end{split}
% \label{eqn:endd-loss1}
% \end{empheq}

%\footnote{From now on, when we refer to Ensemble Distribution Distillation, we explicitly mean Ensemble Distribution Distillation using Dirichlet Prior Networks.}
% \begin{empheq}{align}
% \begin{split} 
% {\tt P}(y = \omega_c| \bm{x}^{*};\bm{\hat \phi}) = &\ \mathbb{E}_{{\tt p}(\bm{\pi} | \bm{x}^{*};\bm{\hat \phi})}[{\tt P}(y = \omega_c | \bm{\pi})]=\ \hat \pi_c =\ \frac{\hat \alpha_c}{\sum_{k=1}^K \hat \alpha_k} =\ \frac{ e^{\hat z_c}}{\sum_{k=1}^K e^{\hat z_k}}
% \end{split}\label{eqn:dirposterior}
% \end{empheq}
% Separable measures of uncertainty can be obtained by considering the mutual information between the prediction $y$ and the parameters of $\bm{\pi}$ of the categorical: 
% \begin{empheq}{align}
% \underbrace{\mathcal{MI}[y,{\tt \bm{\pi}} |\bm{x}^{*};\bm{\hat \phi}]}_{Knowledge\ Uncertainty}=&\ \underbrace{\mathcal{H}\big[\mathbb{E}_{{\tt p}({\tt \bm{\pi}}|\bm{x}^{*};\bm{\hat \phi})}[{\tt P}(y|{\tt \bm{\pi}})]\big]}_{Total\ Uncertainty} - \underbrace{\mathbb{E}_{{\tt p}({\tt \bm{\pi}}|\bm{x}^{*};\bm{\hat \phi})}\big[\mathcal{H}[{\tt P}(y|{\tt \bm{\pi}})]\big]}_{Expected\ Data\ Uncertainty} \label{eqn:mipn}
% \end{empheq}
% Similar to equation~\ref{eqn:mibayes}, this expression allows \emph{total uncertainty}, given by the entropy of the expected distribution, to be decomposed into \emph{data uncertainty} and \emph{knowledge uncertainty}~\citep{malinin-pn-2018}. If Ensemble Distribution Distillation is successful, then the measures of uncertainty derivable from a distribution-distilled model should be identical to those derived from the original ensemble.












% This loss will have the following form in the case of a uni-model Dirichlet:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{L}_{{\tt UD}}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\  -\frac{1}{NB}\sum_{i=1}^N\frac{1}{L_i}\sum_{l=1}^{L_i}\frac{1}{M}\sum_{m=1}^M\ln {\tt Dir}(\bm{\pi}_l^{(im)}|\bm{\hat \alpha}_l^{(i)})
% % \mathcal{L}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\  \frac{1}{NB}\sum_{i=1}^N\frac{1}{L_i}\sum_{l=1}^{L_i}\mathcal{L}(\bm{\phi},\bm{\pi}_l^{(i,1:M)},\bm{y}_{<l}^{(i)},\bm{x}^{(i)}) \\
% % \mathcal{L}(\bm{\phi},\bm{\pi}_l^{(i,1:M)},\bm{y}_{<l}^{(i)},\bm{x}^{(i)}) =&\ -\ln\Gamma(\hat \alpha_{0}^{(i)}) + \sum_{c=1}^K\big[\ln\Gamma(\hat \alpha_{c}^{(i)}) - \frac{1}{M}\sum_{m=1}^M(\hat \alpha_{c}^{(i)} -1)\ln\pi_{c}^{(im)}\big]
% \end{split}
% \label{eqn:endd-loss1}
% \end{empheq}
% In the case of a model which yields a mixture of Dirichlet distributions, the loss is:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{L}_{{\tt MD}}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\ -\frac{1}{NB}\sum_{i=1}^N\frac{1}{L_i}\sum_{l=1}^{L_i}\frac{1}{M}\sum_{m=1}^M\ln \Big[\sum_{j=1}^J w_j^{(il)}{\tt Dir}(\bm{\pi}_l^{(im)}|\bm{\hat \alpha}_l^{(ij)})\Big]
% \end{split}
% \label{eqn:endd-loss2}
% \end{empheq}
% However, due to the sum within the logarithm, it may be difficult to express this loss into a numerically stable way (as we cannot directly take log-gammas). Thus, it may be better to consider minimizing a Jensen-upper bound to this loss:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{L}_{{\tt MD-UB}}(\bm{\phi},\mathcal{D}_{\tt ens}) =&\ -\frac{1}{NB}\sum_{i=1}^N\frac{1}{L_i}\sum_{l=1}^{L_i}\frac{1}{M}\sum_{m=1}^M\sum_{j=1}^J w_j^{(il)}\Big[\ln{\tt Dir}(\bm{\pi}_l^{(im)}|\bm{\hat \alpha}_l^{(i)})\Big] \\
% \geq&\ -\frac{1}{NB}\sum_{i=1}^N\frac{1}{L_i}\sum_{l=1}^{L_i}\frac{1}{M}\sum_{m=1}^M\ln \Big[\sum_{j=1}^J w_j^{(il)}{\tt Dir}(\bm{\pi}_l^{(im)}|\bm{\hat \alpha}_l^{(ij)})\Big] 
% \end{split}
% \label{eqn:endd-loss3}
% \end{empheq}
% As this loss can now be expressed into terms of sums of log-gammas, it can be evaluated with greater numerical stability.

==> structured_uncertainty.tex <==
\section{Uncertainty in Structured Prediction via Ensembles}\label{sec:struct-uncertainty}


% Consider models that capture a mapping $\{x_{1},\cdots,x_T\} = \bm{x} \rightarrow \{y_{1},\cdots,y_L\} = \bm{y}$ between a $T$-length sequence of inputs an $L$-length sequence of targets:
% \begin{empheq}{align}
% {\tt P}(\bm{y}| \bm{x}, \bm{\theta}) =&\ \prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{x}; \bm{\theta})
% \label{eqn:stuct-predict-autoreg}
% \end{empheq}
% In the model above the distribution over each $y_l$ is conditioned on all the previous $\bm{y}_{<l} = \{y_1,\cdots,y_{l-1}\}$, which is called the \emph{context}. These models are typically applied to neural machine translation~\cite{bahdanau2015nmt, attentionisallyouneed}, end-to-end speech recognition \cite{las} and other related tasks. For these models uncertainty estimates can be obtained at two levels - the \emph{token level}, which considers uncertainty in the prediction of a single $y_l$ given a context $\bm{y}_{<l}$ and input $\bm{x}$, and the \emph{sequence level}, which considers the uncertainty of predicting the entire sequence $\bm{y}$ given $\bm{x}$.

% Consider an ensemble of autoregressive models sampled from an approximate posterior ${\tt q}(\bm{\theta})$
% \begin{empheq}{align}
% \{{\tt P}(\bm{y} | \bm{x}; \bm{\theta}^{(m)})\}_{m=1}^M\  \bm{\theta}^{(m)} \sim {\tt q}(\bm{\theta}) \approx {\tt p}(\bm{\theta}|\mathcal{D})
% \label{eqn:stuct-predict-autoreg}
% \end{empheq}
% Given this ensemble we can expressive the predictive posterior either as \emph{sequence-level} Bayesian Model Averaging (BMA) or \emph{token-level} BMA. The former assumes that each sequence $\bm{y}$ has been generated by a \emph{particular} $\bm{\theta}^{(m)}$, as follows:
% \begin{empheq}{align}
% \begin{split}
% {\tt P}(\bm{y}|  \bm{x}, \mathcal{D}) =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(\bm{y}| \bm{x},  \bm{\theta})\Big]
%                              \ \ =\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \bm{\theta}) \Big]
% \end{split}\label{eqn:expectation-of-products}
% \end{empheq}
% On the other hand, token-level BMA assumes that a particular model $\bm{\theta}^{(m)}$ yields only a particular token $y_l$, and other tokens could haven been generated by other models in the ensemble:
% \begin{empheq}{align}
% \begin{split}
% {\tt P}(\bm{y}|  \bm{x}, \mathcal{D}) =&\  \prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \mathcal{D})
%                              =\ \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \bm{\theta})\Big] 
% \end{split}\label{eqn:product-of-expectations}
% \end{empheq}
% Intuitively, it would seem that sequence-level BMA is more appropriate for both model combination and uncertainty estimation in structured prediction. However, it was shown in ~\cite{malinin-structured-2020}, a token-level BMA consistently yields better predictive performance in terms of BLEU and WER, lower negative log-likelihoods on the reference transcriptions and marginally more informative uncertainty estimates than sequence-level BMA. In fact, this result was consistent across all tasks, ensemble sizes and dataset sizes. 

In this section we describe ensemble-based uncertainty estimation for structured prediction. Consider models that capture a mapping $\{\bm{x}_{1},\cdots,\bm{x}_T\} \rightarrow \{y_{1},\cdots,y_L\}$ between a $T$-length sequence of inputs $\{\bm{x}_1,\cdots,\bm{x}_T\} = \bm{x}$ and an $L$-length sequence of targets $\{y_1,\cdots,y_L\} = \bm{y}$, where the targets $\bm{y}$ are auto-regressive:
\begin{empheq}{align}
{\tt P}(\bm{y}| \bm{x}, \bm{\theta}) =&\  \prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{x}; \bm{\theta})
\label{eqn:stuct-predict-autoreg}
\end{empheq}
In the model above the distribution over each $y_l$ is conditioned on all the previous $\bm{y}_{<l} = \{y_1,\cdots,y_{l-1}\}$, which is called the \emph{context}. These models are typically applied to neural machine translation~\cite{bahdanau2015nmt, attentionisallyouneed}, end-to-end speech recognition \cite{las} and other related tasks. For these models uncertainty estimates can be obtained at two levels - the \emph{token level}, which considers uncertainty in the prediction of a single $y_l$ given a context $\bm{y}_{<l}$ and input $\bm{x}$, and the \emph{sequence level}, which considers the uncertainty of predicting the entire sequence $\bm{y}$ given $\bm{x}$.

Here, we consider ensembles of auto-regressive models sampled from an approximate Bayesian posterior ${\tt q}(\bm{\theta})$:
\begin{empheq}{align}
\big\{ {\tt P}(y_l | \bm{y}_{<l}, \bm{x}; \bm{\theta}^{(m)}) \big\}_{m=1}^M,\  \bm{\theta}^{(m)} \sim {\tt q}(\bm{\theta}) \approx {\tt p}(\bm{\theta}|\mathcal{D})
\label{eqn:stuct-predict-autoreg}
\end{empheq}
Given this ensemble, the predictive posterior can be obtained either as a product of expectations:
\begin{empheq}{align}
{\tt P}_{\tt S-BMA}(\bm{y}|  \bm{x}, \mathcal{D}) =&\  \prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \mathcal{D})
                             =\ \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \bm{\theta})\Big] \label{eqn:product-of-expectations} \\
{\tt P}_{\tt T-BMA}(\bm{y}|  \bm{x}, \mathcal{D}) =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(\bm{y}| \bm{x},  \bm{\theta})\Big]
                             \ \ =\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l},  \bm{x}, \bm{\theta}) \Big] \label{eqn:expectation-of-products}
\end{empheq}
As was shown in ~\cite{malinin-structured-2020}, combining the model as a product of expectations consistently yields better BLEU and WER scores as well as better log-likelihoods on the reference transcriptions. Thus, in this work only ensembles combined as a product-of-expectations are considered.
